New Planar P-time Computable Six-Vertex Models and a Complete Complexity Classification

We discover new P-time computable six-vertex models on planar graphs beyond Kasteleyn's algorithm for counting planar perfect matchings. We further prove that there are no more: Together, they exhaust all P-time computable six-vertex models on planar graphs, assuming #P is not P. This leads to the following exact complexity classification: For every parameter setting in ${\mathbb C}$ for the six-vertex model, the partition function is either (1) computable in P-time for every graph, or (2) #P-hard for general graphs but computable in P-time for planar graphs, or (3) #P-hard even for planar graphs. The classification has an explicit criterion. The new P-time cases in (2) provably cannot be subsumed by Kasteleyn's algorithm. They are obtained by a non-local connection to #CSP, defined in terms of a "loop space". This is the first substantive advance toward a planar Holant classification with not necessarily symmetric constraints. We introduce M�\"obius transformation on ${\mathbb C}$ as a powerful new tool in hardness proofs for counting problems.

==> bmod-occure <==
preliminaries.tex:For any assignment in those categories with parameters $(i, j, k)$ where $k \equiv 0 (\bmod ~2)$, the evaluation of
preliminaries.tex:$(M(f_{2s+1}))^{\otimes m}$ is clearly $(-1)^kb^{(2s+1)j}=b^{(2s+1)j}$. And for any assignment in those categories with parameters $(i, j, k)$ where $k \equiv 1 (\bmod~2)$, the evaluation of
preliminaries.tex:Since $i+j+k=m$, the index $i$ is determined by $j$ and $k$. Let $a_{j0}$ be the summation of values of the part $A$ over all assignments in those categories $(i, j, k)$ where $k \equiv 0 (\bmod ~2)$, and $a_{j1}$ be the summation of values of the part $A$ over all assignments in those categories $(i, j, k)$ where $k \equiv 1 (\bmod ~2)$. %Since $i+j+k=m$, we can denote $a_{ij0}$ by $a_{j0}$ and $a_{ij1}$ by $a_{j1}$. 
preliminaries.tex:%\end{smallmatrix}\right]$, where $q_{00}, q_{01}, q_{10}, q_{11} \in \mathbb{N}$ and $q_{00}+q_{01}+q_{10}+q_{11} \equiv 0 (\bmod ~2)$. 
twozero.tex:Since $G$ is a planar graph, $|V_{i, j}| \equiv 0 ~(\bmod ~2).$ 
twozero.tex:%Since $G$ is a planar graph, $|V_{i, j}| \equiv 0 ~(\bmod 2).$ 
twozero.tex:%We get a set of $k+l$ intersection vertices in $D_1$ and $D_2$, denoted by $V_{12}$. Since $k+l\equiv 0 ~(\bmod 2)$, $|V_{12}| \equiv 0 ~(\bmod 2)$.
twozero.tex: %We get vertices sets $U_j$, $V_{1j}$, $\cdots$, $V_{(j-1) i}$ and $|V_{i, j}|\equiv 0 ~(\bmod 2)$.
twozero.tex:Since $\bar{G}$ is a planar graph, $|\bar{V}_{ij}| \equiv 0 ~(\bmod 2)$. We already know $|V_{i, j}| \equiv 0 ~(\bmod 2)$, so $|\bar{V}_{ij}\backslash V_{i, j}|=|\bar{V}_{ij}|-|V_{i, j}| \equiv 0 ~(\bmod 2)$. 
twozero.tex:\item[$\operatorname{(\rmnum{2})}$.] $x=a\frak{i}^\alpha, b=a\sqrt{\frak{i}}^\beta, y=a\sqrt{\frak{i}}^\gamma$, where $\alpha, \beta, \gamma \in \mathbb{N}$, and $\beta\equiv \gamma ~(\bmod ~2),$
twozero.tex:%Since $o-e \equiv k+l \equiv 0 ~(\bmod 2)$, 
twozero.tex:Since $(k_1+\ell_1+k_3+\ell_3)-(k_2+\ell_2+k_4+\ell_4)\equiv k+\ell \equiv 0 ~(\bmod ~2)$, 
twozero.tex: Since $\beta\equiv \gamma ~(\bmod~2)$, if they are both even, 
twozero.tex: then $p_{00} \equiv p_{01} \equiv p_{10} \equiv p_{11} \equiv 0 ~(\bmod ~2);$ 
twozero.tex: p_{01} \equiv p_{10} ~(\bmod ~2).$ 
twozero.tex: Hence, $g$ is of the form $a'(\frak{i}^{q_{00}}, \frak{i}^{q_{01}}, \frak{i}^{q_{10}}, \frak{i}^{q_{11}})^T$, where $a'=a^{k+l}$ or $a^{k+l}\sqrt{\frak{i}}$, and for all $i, j \in \{0, 1\}$, $q_{ij}=\frac{p_{ij}}{2}$ or $\frac{p_{ij}-1}{2}$. Thus, $$q_{00}+q_{01}+q_{10}+q_{11} \equiv (p_{00} + p_{01} + p_{10} + p_{11})/2  ~(\bmod ~2).$$ 
twozero.tex: Moreover, since $p_{00} + p_{01} + p_{10} + p_{11}=(k+\ell)(\beta+\gamma+2\alpha) \equiv 0 ~(\bmod ~4),$ we have $q_{00}+q_{01}+q_{10}+q_{11} \equiv 0 ~(\bmod ~2)$.
twozero.tex:Since $\beta \equiv \gamma  ~(\bmod~2)$, we have $\beta m_2+\gamma m_4 \equiv \beta m_4+\gamma m_2 ~(\bmod ~2)$. Hence, $h$ is of the form $a'^\prime(i^{q_0}, i^{q_1})$, where $a''=a^{m}$ or $a^{m}\sqrt{\frak{i}}$. That is, $h \in \mathscr{A}$ by Lemma \ref{2affine}. Hence, $\mathcal{G}_f\cup \mathcal{H}_f \subseteq \mathscr{A}$. 
twozero.tex:Also, since $g_{1_f}\in \mathscr{A}$, $b^{\prime}y^{\prime}=\sqrt{\ii}^{\beta+\gamma}$ is a power of $\ii$, which means $\beta\equiv \gamma ~(\bmod ~2).$ That is, $\{a, b, x, y\}$ belongs to case (\rmnum{2}).
twozero.tex:%Also since $b^{\prime}y^{\prime}$ is power of $i$, we have $B\equiv Y %(\bmod 2).$ That is, $a, b, x, y$ belong to case (\rmnum{2}). %Contradiction. 

